AnyMAL: An Efficient and Scalable Any-Modality Augmented Language Model

We present Any-Modality Augmented Language Model (AnyMAL), a unified model that reasons over diverse input modality signals (i.e. text, image, video, audio, IMU motion sensor), and generates textual responses. AnyMAL inherits the powerful text-based reasoning abilities of the state-of-the-art LLMs including LLaMA-2 (70B), and converts modality-specific signals to the joint textual space through a pre-trained aligner module. To further strengthen the multimodal LLM's capabilities, we fine-tune the model with a multimodal instruction set manually collected to cover diverse topics and tasks beyond simple QAs. We conduct comprehensive empirical analysis comprising both human and automatic evaluations, and demonstrate state-of-the-art performance on various multimodal tasks.

==> bbl_20230927.tex <==
\begin{thebibliography}{10}

\bibitem{tsimpoukelli2021multimodal}
M.~Tsimpoukelli, J.~L. Menick, S.~Cabi, S.~Eslami, O.~Vinyals, and F.~Hill,
  ``Multimodal few-shot learning with frozen language models,'' {\em Advances
  in Neural Information Processing Systems}, vol.~34, pp.~200--212, 2021.

\bibitem{flamingo}
J.-B. Alayrac, J.~Donahue, P.~Luc, A.~Miech, I.~Barr, Y.~Hasson, K.~Lenc,
  A.~Mensch, K.~Millican, M.~Reynolds, {\em et~al.}, ``Flamingo: a visual
  language model for few-shot learning,'' {\em Advances in Neural Information
  Processing Systems}, vol.~35, pp.~23716--23736, 2022.

\bibitem{blip2}
J.~Li, D.~Li, S.~Savarese, and S.~Hoi, ``Blip-2: Bootstrapping language-image
  pre-training with frozen image encoders and large language models,'' {\em
  arXiv preprint arXiv:2301.12597}, 2023.

\bibitem{OpenAI2023GPT4TR}
OpenAI, ``Gpt-4 technical report,'' {\em ArXiv}, vol.~abs/2303.08774, 2023.

\bibitem{idefics}
H.~Laurençon, L.~Saulnier, L.~Tronchon, S.~Bekman, A.~Singh, A.~Lozhkov,
  T.~Wang, S.~Karamcheti, A.~M. Rush, D.~Kiela, M.~Cord, and V.~Sanh,
  ``Obelics: An open web-scale filtered dataset of interleaved image-text
  documents,'' 2023.

\bibitem{llama2}
H.~Touvron, L.~Martin, K.~Stone, P.~Albert, A.~Almahairi, Y.~Babaei,
  N.~Bashlykov, S.~Batra, P.~Bhargava, S.~Bhosale, {\em et~al.}, ``Llama 2:
  Open foundation and fine-tuned chat models,'' {\em arXiv preprint
  arXiv:2307.09288}, 2023.

\bibitem{GPT2}
A.~Radford, J.~Wu, R.~Child, D.~Luan, D.~Amodei, I.~Sutskever, {\em et~al.},
  ``Language models are unsupervised multitask learners,'' 2019.

\bibitem{flant5}
H.~W. Chung, L.~Hou, S.~Longpre, B.~Zoph, Y.~Tay, W.~Fedus, E.~Li, X.~Wang,
  M.~Dehghani, S.~Brahma, A.~Webson, S.~S. Gu, Z.~Dai, M.~Suzgun, X.~Chen,
  A.~Chowdhery, S.~Narang, G.~Mishra, A.~Yu, V.~Zhao, Y.~Huang, A.~Dai, H.~Yu,
  S.~Petrov, E.~H. Chi, J.~Dean, J.~Devlin, A.~Roberts, D.~Zhou, Q.~V. Le, and
  J.~Wei, ``Scaling instruction-finetuned language models,'' 2022.

\bibitem{gpt-j}
B.~Wang and A.~Komatsuzaki, ``{GPT-J-6B: A 6 Billion Parameter Autoregressive
  Language Model}.'' \url{https://github.com/kingoflolz/mesh-transformer-jax},
  May 2021.

\bibitem{opt}
S.~Zhang, S.~Roller, N.~Goyal, M.~Artetxe, M.~Chen, S.~Chen, C.~Dewan, M.~Diab,
  X.~Li, X.~V. Lin, {\em et~al.}, ``Opt: Open pre-trained transformer language
  models,'' {\em arXiv preprint arXiv:2205.01068}, 2022.

\bibitem{llama}
H.~Touvron, T.~Lavril, G.~Izacard, X.~Martinet, M.-A. Lachaux, T.~Lacroix,
  B.~Rozi{\`e}re, N.~Goyal, E.~Hambro, F.~Azhar, {\em et~al.}, ``Llama: Open
  and efficient foundation language models,'' {\em arXiv preprint
  arXiv:2302.13971}, 2023.

\bibitem{vicuna}
W.-L. Chiang, Z.~Li, Z.~Lin, Y.~Sheng, Z.~Wu, H.~Zhang, L.~Zheng, S.~Zhuang,
  Y.~Zhuang, J.~E. Gonzalez, I.~Stoica, and E.~P. Xing, ``Vicuna: An
  open-source chatbot impressing gpt-4 with 90\%* chatgpt quality,'' March
  2023.

\bibitem{xu2015show}
K.~Xu, J.~Ba, R.~Kiros, K.~Cho, A.~Courville, R.~Salakhudinov, R.~Zemel, and
  Y.~Bengio, ``Show, attend and tell: Neural image caption generation with
  visual attention,'' in {\em International conference on machine learning},
  pp.~2048--2057, PMLR, 2015.

\bibitem{vqa}
S.~Antol, A.~Agrawal, J.~Lu, M.~Mitchell, D.~Batra, C.~Lawrence~Zitnick, and
  D.~Parikh, ``{VQA}: Visual question answering,'' in {\em ICCV}, 2015.

\bibitem{visdial}
A.~Das, S.~Kottur, K.~Gupta, A.~Singh, D.~Yadav, J.~M. Moura, D.~Parikh, and
  D.~Batra, ``Visual dialog,'' in {\em CVPR}, 2017.

\bibitem{vision-language-navigation}
P.~Anderson, Q.~Wu, D.~Teney, J.~Bruce, M.~Johnson, N.~S{\"u}nderhauf, I.~Reid,
  S.~Gould, and A.~van~den Hengel, ``Vision-and-language navigation:
  Interpreting visually-grounded navigation instructions in real
  environments,'' in {\em Proceedings of the IEEE Conference on Computer Vision
  and Pattern Recognition}, pp.~3674--3683, 2018.

\bibitem{openflamingo}
A.~Awadalla, I.~Gao, J.~Gardner, J.~Hessel, Y.~Hanafy, W.~Zhu, K.~Marathe,
  Y.~Bitton, S.~Gadre, J.~Jitsev, S.~Kornblith, P.~W. Koh, G.~Ilharco,
  M.~Wortsman, and L.~Schmidt, ``Openflamingo,'' Mar. 2023.

\bibitem{palme}
D.~Driess, F.~Xia, M.~S.~M. Sajjadi, C.~Lynch, A.~Chowdhery, B.~Ichter,
  A.~Wahid, J.~Tompson, Q.~Vuong, T.~Yu, W.~Huang, Y.~Chebotar, P.~Sermanet,
  D.~Duckworth, S.~Levine, V.~Vanhoucke, K.~Hausman, M.~Toussaint, K.~Greff,
  A.~Zeng, I.~Mordatch, and P.~Florence, ``Palm-e: An embodied multimodal
  language model,'' in {\em arXiv preprint arXiv:2303.03378}, 2023.

\bibitem{instructblip}
W.~Dai, J.~Li, D.~Li, A.~M.~H. Tiong, J.~Zhao, W.~Wang, B.~Li, P.~Fung, and
  S.~Hoi, ``Instructblip: Towards general-purpose vision-language models with
  instruction tuning,'' 2023.

\bibitem{llava}
H.~Liu, C.~Li, Q.~Wu, and Y.~J. Lee, ``Visual instruction tuning,'' 2023.

\bibitem{minigpt4}
D.~Zhu, J.~Chen, X.~Shen, X.~Li, and M.~Elhoseiny, ``Minigpt-4: Enhancing
  vision-language understanding with advanced large language models,'' {\em
  arXiv preprint arXiv:2304.10592}, 2023.

\bibitem{otter}
B.~Li, Y.~Zhang, L.~Chen, J.~Wang, J.~Yang, and Z.~Liu, ``Otter: A multi-modal
  model with in-context instruction tuning,'' {\em arXiv preprint
  arXiv:2305.03726}, 2023.

\bibitem{mplug}
Q.~Ye, H.~Xu, G.~Xu, J.~Ye, M.~Yan, Y.~Zhou, J.~Wang, A.~Hu, P.~Shi, Y.~Shi,
  {\em et~al.}, ``mplug-owl: Modularization empowers large language models with
  multimodality,'' {\em arXiv preprint arXiv:2304.14178}, 2023.

\bibitem{multimodalGPT}
T.~Gong, C.~Lyu, S.~Zhang, Y.~Wang, M.~Zheng, Q.~Zhao, K.~Liu, W.~Zhang,
  P.~Luo, and K.~Chen, ``Multimodal-gpt: A vision and language model for
  dialogue with humans,'' {\em arXiv preprint arXiv:2305.04790}, 2023.

\bibitem{lamaadapterv2}
P.~Gao, J.~Han, R.~Zhang, Z.~Lin, S.~Geng, A.~Zhou, W.~Zhang, P.~Lu, C.~He,
  X.~Yue, H.~Li, and Y.~Qiao, ``Llama-adapter v2: Parameter-efficient visual
  instruction model,'' {\em arXiv preprint arXiv:2304.15010}, 2023.

\bibitem{zhang2023video}
H.~Zhang, X.~Li, and L.~Bing, ``Video-llama: An instruction-tuned audio-visual
  language model for video understanding,'' {\em arXiv preprint
  arXiv:2306.02858}, 2023.

\bibitem{su2023pandagpt}
Y.~Su, T.~Lan, H.~Li, J.~Xu, Y.~Wang, and D.~Cai, ``Pandagpt: One model to
  instruction-follow them all,'' {\em arXiv preprint arXiv:2305.16355}, 2023.

\bibitem{lyu2023macaw}
C.~Lyu, M.~Wu, L.~Wang, X.~Huang, B.~Liu, Z.~Du, S.~Shi, and Z.~Tu,
  ``Macaw-llm: Multi-modal language modeling with image, audio, video, and text
  integration,'' {\em arXiv preprint arXiv:2306.09093}, 2023.

\bibitem{m3it}
L.~Li, Y.~Yin, S.~Li, L.~Chen, P.~Wang, S.~Ren, M.~Li, Y.~Yang, J.~Xu, X.~Sun,
  {\em et~al.}, ``Mit: A large-scale dataset towards multi-modal multilingual
  instruction tuning,'' {\em arXiv preprint arXiv:2306.04387}, 2023.

\bibitem{clip}
A.~Radford, J.~W. Kim, C.~Hallacy, A.~Ramesh, G.~Goh, S.~Agarwal, G.~Sastry,
  A.~Askell, P.~Mishkin, J.~Clark, {\em et~al.}, ``Learning transferable visual
  models from natural language supervision,'' in {\em International Conference
  on Machine Learning (ICML)}, 2021.

\bibitem{laion}
C.~Schuhmann, R.~Beaumont, R.~Vencu, C.~Gordon, R.~Wightman, M.~Cherti,
  T.~Coombes, A.~Katta, C.~Mullis, M.~Wortsman, {\em et~al.}, ``Laion-5b: An
  open large-scale dataset for training next generation image-text models,''
  {\em Advances in Neural Information Processing Systems}, vol.~35,
  pp.~25278--25294, 2022.

\bibitem{clap}
Y.~Wu*, K.~Chen*, T.~Zhang*, Y.~Hui*, T.~Berg-Kirkpatrick, and S.~Dubnov,
  ``Large-scale contrastive language-audio pretraining with feature fusion and
  keyword-to-caption augmentation,'' in {\em IEEE International Conference on
  Acoustics, Speech and Signal Processing, ICASSP}, 2023.

\bibitem{imu2clip}
S.~Moon, A.~Madotto, Z.~Lin, A.~Dirafzoon, A.~Saraf, A.~Bearman, and
  B.~Damavandi, ``Imu2clip: Multimodal contrastive learning for imu motion
  sensors from egocentric videos and text,'' {\em arXiv preprint
  arXiv:2210.14395}, 2022.

\bibitem{laionfiltering}
F.~Radenovic, A.~Dubey, A.~Kadian, T.~Mihaylov, S.~Vandenhende, Y.~Patel,
  Y.~Wen, V.~Ramanathan, and D.~Mahajan, ``Filtering, distillation, and hard
  negatives for vision-language pre-training,'' in {\em Proceedings of the
  IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pp.~6967--6977, 2023.

\bibitem{audioset}
J.~F. Gemmeke, D.~P.~W. Ellis, D.~Freedman, A.~Jansen, W.~Lawrence, R.~C.
  Moore, M.~Plakal, and M.~Ritter, ``Audio set: An ontology and human-labeled
  dataset for audio events,'' in {\em Proc. IEEE ICASSP 2017}, (New Orleans,
  LA), 2017.

\bibitem{kim2019audiocaps}
C.~D. Kim, B.~Kim, H.~Lee, and G.~Kim, ``Audiocaps: Generating captions for
  audios in the wild,'' in {\em Proceedings of the 2019 Conference of the North
  American Chapter of the Association for Computational Linguistics: Human
  Language Technologies, Volume 1 (Long and Short Papers)}, pp.~119--132, 2019.

\bibitem{clotho}
K.~Drossos, S.~Lipping, and T.~Virtanen, ``Clotho: An audio captioning
  dataset,'' in {\em ICASSP 2020-2020 IEEE International Conference on
  Acoustics, Speech and Signal Processing (ICASSP)}, pp.~736--740, IEEE, 2020.

\bibitem{ego4d}
K.~Grauman, A.~Westbury, E.~Byrne, Z.~Chavis, A.~Furnari, R.~Girdhar,
  J.~Hamburger, H.~Jiang, M.~Liu, X.~Liu, M.~Martin, T.~Nagarajan,
  I.~Radosavovic, S.~K. Ramakrishnan, F.~Ryan, J.~Sharma, M.~Wray, M.~Xu, E.~Z.
  Xu, C.~Zhao, S.~Bansal, D.~Batra, V.~Cartillier, S.~Crane, T.~Do, M.~Doulaty,
  A.~Erapalli, C.~Feichtenhofer, A.~Fragomeni, Q.~Fu, C.~Fuegen,
  A.~Gebreselasie, C.~Gonzalez, J.~Hillis, X.~Huang, Y.~Huang, W.~Jia, W.~Khoo,
  J.~Kolar, S.~Kottur, A.~Kumar, F.~Landini, C.~Li, Y.~Li, Z.~Li, K.~Mangalam,
  R.~Modhugu, J.~Munro, T.~Murrell, T.~Nishiyasu, W.~Price, P.~R. Puentes,
  M.~Ramazanova, L.~Sari, K.~Somasundaram, A.~Southerland, Y.~Sugano, R.~Tao,
  M.~Vo, Y.~Wang, X.~Wu, T.~Yagi, Y.~Zhu, P.~Arbelaez, D.~Crandall, D.~Damen,
  G.~M. Farinella, B.~Ghanem, V.~K. Ithapu, C.~V. Jawahar, H.~Joo, K.~Kitani,
  H.~Li, R.~Newcombe, A.~Oliva, H.~S. Park, J.~M. Rehg, Y.~Sato, J.~Shi, M.~Z.
  Shou, A.~Torralba, L.~Torresani, M.~Yan, and J.~Malik, ``Ego4d: Around the
  {W}orld in 3,000 {H}ours of {E}gocentric {V}ideo,'' in {\em IEEE/CVF Computer
  Vision and Pattern Recognition (CVPR)}, 2022.

\bibitem{zhao2023pytorch}
Y.~Zhao, A.~Gu, R.~Varma, L.~Luo, C.-C. Huang, M.~Xu, L.~Wright,
  H.~Shojanazeri, M.~Ott, S.~Shleifer, A.~Desmaison, C.~Balioglu, P.~Damania,
  B.~Nguyen, G.~Chauhan, Y.~Hao, A.~Mathews, and S.~Li, ``Pytorch fsdp:
  Experiences on scaling fully sharded data parallel,'' 2023.

\bibitem{qlora}
T.~Dettmers, A.~Pagnoni, A.~Holtzman, and L.~Zettlemoyer, ``Qlora: Efficient
  finetuning of quantized llms,'' {\em arXiv preprint arXiv:2305.14314}, 2023.

\bibitem{lora}
E.~J. Hu, Y.~Shen, P.~Wallis, Z.~Allen-Zhu, Y.~Li, S.~Wang, L.~Wang, and
  W.~Chen, ``Lora: Low-rank adaptation of large language models,'' {\em arXiv
  preprint arXiv:2106.09685}, 2021.

\bibitem{cm3leon}
L.~Yu, B.~Shi, R.~Pasunuru, B.~Miller, O.~Golovneva, T.~Wang, A.~Babu, B.~Tang,
  B.~Karrer, S.~Sheynin, C.~Ross, A.~Polyak, R.~Howes, V.~Sharma, J.~Xu,
  U.~Singer, D.~Li, G.~Ghosh, Y.~Taigman, M.~Fazel-Zarandi, A.~Celikyilmaz,
  L.~Zettlemoyer, and A.~Aghajanyan, ``Scaling autoregressive multi-modal
  models: Pretraining and instruction tuning,'' 2023.

\bibitem{xu2021investigating}
X.~Xu, H.~Dinkel, M.~Wu, Z.~Xie, and K.~Yu, ``Investigating local and global
  information for automated audio captioning with transfer learning,'' in {\em
  ICASSP 2021-2021 IEEE International Conference on Acoustics, Speech and
  Signal Processing (ICASSP)}, pp.~905--909, IEEE, 2021.

\bibitem{mei2021audio}
X.~Mei, X.~Liu, Q.~Huang, M.~D. Plumbley, and W.~Wang, ``Audio captioning
  transformer,'' {\em arXiv preprint arXiv:2107.09817}, 2021.

\bibitem{liu2022leveraging}
X.~Liu, X.~Mei, Q.~Huang, J.~Sun, J.~Zhao, H.~Liu, M.~D. Plumbley, V.~Kilic,
  and W.~Wang, ``Leveraging pre-trained bert for audio captioning,'' in {\em
  2022 30th European Signal Processing Conference (EUSIPCO)}, pp.~1145--1149,
  IEEE, 2022.

\bibitem{wang2022internvideo}
Y.~Wang, K.~Li, Y.~Li, Y.~He, B.~Huang, Z.~Zhao, H.~Zhang, J.~Xu, Y.~Liu,
  Z.~Wang, {\em et~al.}, ``Internvideo: General video foundation models via
  generative and discriminative learning,'' {\em arXiv preprint
  arXiv:2212.03191}, 2022.

\bibitem{li2023blip}
J.~Li, D.~Li, S.~Savarese, and S.~Hoi, ``Blip-2: Bootstrapping language-image
  pre-training with frozen image encoders and large language models,'' {\em
  arXiv preprint arXiv:2301.12597}, 2023.

\bibitem{mscoco}
T.-Y. Lin, M.~Maire, S.~Belongie, J.~Hays, P.~Perona, D.~Ramanan,
  P.~Doll{\'a}r, and C.~L. Zitnick, ``Microsoft coco: Common objects in
  context,'' in {\em ECCV}, 2014.

\bibitem{hatefulmeme}
D.~Kiela, H.~Firooz, A.~Mohan, V.~Goswami, A.~Singh, P.~Ringshia, and
  D.~Testuggine, ``The hateful memes challenge: Detecting hate speech in
  multimodal memes,'' {\em Advances in neural information processing systems},
  vol.~33, pp.~2611--2624, 2020.

\bibitem{TextVQA}
A.~Singh, V.~Natarjan, M.~Shah, Y.~Jiang, X.~Chen, D.~Parikh, and M.~Rohrbach,
  ``Towards vqa models that can read,'' in {\em Proceedings of the IEEE
  Conference on Computer Vision and Pattern Recognition}, pp.~8317--8326, 2019.

\bibitem{scienceqa}
P.~Lu, S.~Mishra, T.~Xia, L.~Qiu, K.-W. Chang, S.-C. Zhu, O.~Tafjord, P.~Clark,
  and A.~Kalyan, ``Learn to explain: Multimodal reasoning via thought chains
  for science question answering,'' {\em Advances in Neural Information
  Processing Systems}, vol.~35, pp.~2507--2521, 2022.

\bibitem{vizwiz}
D.~Gurari, Q.~Li, A.~J. Stangl, A.~Guo, C.~Lin, K.~Grauman, J.~Luo, and J.~P.
  Bigham, ``Vizwiz grand challenge: Answering visual questions from blind
  people,'' in {\em Proceedings of the IEEE conference on computer vision and
  pattern recognition}, pp.~3608--3617, 2018.

\bibitem{okvqa}
K.~Marino, M.~Rastegari, A.~Farhadi, and R.~Mottaghi, ``Ok-vqa: A visual
  question answering benchmark requiring external knowledge,'' in {\em
  Proceedings of the IEEE/cvf conference on computer vision and pattern
  recognition}, pp.~3195--3204, 2019.

\bibitem{dinov2}
M.~Oquab, T.~Darcet, T.~Moutakanni, H.~V. Vo, M.~Szafraniec, V.~Khalidov,
  P.~Fernandez, D.~Haziza, F.~Massa, A.~El-Nouby, R.~Howes, P.-Y. Huang, H.~Xu,
  V.~Sharma, S.-W. Li, W.~Galuba, M.~Rabbat, M.~Assran, N.~Ballas, G.~Synnaeve,
  I.~Misra, H.~Jegou, J.~Mairal, P.~Labatut, A.~Joulin, and P.~Bojanowski,
  ``Dinov2: Learning robust visual features without supervision,'' 2023.

\bibitem{li2020hero}
L.~Li, Y.-C. Chen, Y.~Cheng, Z.~Gan, L.~Yu, and J.~Liu, ``Hero: Hierarchical
  encoder for video+ language omni-representation pre-training,'' {\em arXiv
  preprint arXiv:2005.00200}, 2020.

\bibitem{wu2021star}
B.~Wu, S.~Yu, Z.~Chen, J.~B. Tenenbaum, and C.~Gan, ``Star: A benchmark for
  situated reasoning in real-world videos,'' in {\em Thirty-fifth Conference on
  Neural Information Processing Systems Datasets and Benchmarks Track (Round
  2)}, 2021.

\bibitem{xiao2021next}
J.~Xiao, X.~Shang, A.~Yao, and T.-S. Chua, ``Next-qa: Next phase of
  question-answering to explaining temporal actions,'' in {\em Proceedings of
  the IEEE/CVF conference on computer vision and pattern recognition},
  pp.~9777--9786, 2021.

\bibitem{yu2023self}
S.~Yu, J.~Cho, P.~Yadav, and M.~Bansal, ``Self-chained image-language model for
  video localization and question answering,'' {\em arXiv preprint
  arXiv:2305.06988}, 2023.

\bibitem{miech2019howto100m}
A.~Miech, D.~Zhukov, J.-B. Alayrac, M.~Tapaswi, I.~Laptev, and J.~Sivic,
  ``Howto100m: Learning a text-video embedding by watching hundred million
  narrated video clips,'' in {\em Proceedings of the IEEE/CVF international
  conference on computer vision}, pp.~2630--2640, 2019.

\bibitem{radosavovic2020designing}
I.~Radosavovic, R.~P. Kosaraju, R.~Girshick, K.~He, and P.~Dollár, ``Designing
  network design spaces,'' 2020.

\bibitem{roberta}
Y.~Liu, M.~Ott, N.~Goyal, J.~Du, M.~Joshi, D.~Chen, O.~Levy, M.~Lewis,
  L.~Zettlemoyer, and V.~Stoyanov, ``Roberta: A robustly optimized bert
  pretraining approach,'' {\em arXiv preprint arXiv:1907.11692}, 2019.

\bibitem{singer2022make}
U.~Singer, A.~Polyak, T.~Hayes, X.~Yin, J.~An, S.~Zhang, Q.~Hu, H.~Yang,
  O.~Ashual, O.~Gafni, {\em et~al.}, ``Make-a-video: Text-to-video generation
  without text-video data,'' {\em arXiv preprint arXiv:2209.14792}, 2022.

\bibitem{rlhf}
P.~F. Christiano, J.~Leike, T.~Brown, M.~Martic, S.~Legg, and D.~Amodei, ``Deep
  reinforcement learning from human preferences,'' {\em Advances in neural
  information processing systems}, vol.~30, 2017.

\bibitem{bai2022constitutional}
Y.~Bai, S.~Kadavath, S.~Kundu, A.~Askell, J.~Kernion, A.~Jones, A.~Chen,
  A.~Goldie, A.~Mirhoseini, C.~McKinnon, {\em et~al.}, ``Constitutional ai:
  Harmlessness from ai feedback,'' {\em arXiv preprint arXiv:2212.08073}, 2022.

\bibitem{dpo}
R.~Rafailov, A.~Sharma, E.~Mitchell, S.~Ermon, C.~D. Manning, and C.~Finn,
  ``Direct preference optimization: Your language model is secretly a reward
  model,'' {\em arXiv preprint arXiv:2305.18290}, 2023.

\bibitem{transformers}
T.~Wolf, L.~Debut, V.~Sanh, J.~Chaumond, C.~Delangue, A.~Moi, P.~Cistac,
  T.~Rault, R.~Louf, M.~Funtowicz, J.~Davison, S.~Shleifer, P.~von Platen,
  C.~Ma, Y.~Jernite, J.~Plu, C.~Xu, T.~L. Scao, S.~Gugger, M.~Drame, Q.~Lhoest,
  and A.~M. Rush, ``Transformers: State-of-the-art natural language
  processing,'' in {\em Proceedings of the 2020 Conference on Empirical Methods
  in Natural Language Processing: System Demonstrations}, Oct. 2020.

\bibitem{pytorch}
A.~Paszke, S.~Gross, F.~Massa, A.~Lerer, J.~Bradbury, G.~Chanan, T.~Killeen,
  Z.~Lin, N.~Gimelshein, L.~Antiga, A.~Desmaison, A.~Kopf, E.~Yang, Z.~DeVito,
  M.~Raison, A.~Tejani, S.~Chilamkurthy, B.~Steiner, L.~Fang, J.~Bai, and
  S.~Chintala, ``Pytorch: An imperative style, high-performance deep learning
  library,'' in {\em Neural Information Processing Systems}, 2019.

\end{thebibliography}


==> sections/abstract_plain.tex <==
We present Any-Modality Augmented Language Model (AnyMAL), a unified model that reasons over diverse input modality signals (i.e. text, image, video, audio, IMU), and generates textual responses.
AnyMAL inherits the powerful text-based reasoning abilities of the state-of-the-art LLMs including LLaMA-2 (70B), and converts modality-specific signals to the joint textual space through a pre-trained aligner module.
To further strengthen the multimodal LLM's capabilities, we fine-tune the model with a multimodal instruction set manually collected to cover diverse topics and tasks beyond simple QAs.
We conduct comprehensive empirical analysis comprising both human and automatic evaluations, and demonstrate state-of-the-art performance on various multimodal tasks.

==> sections/archive.tex <==
To measure if the \mn response is relevant and correct with respect to the query and the image, we use the following rubrics to collect human feedback data.

\noindent \textbf{Recognition Accuracy}: Did the model correctly understand and identify the objects or scenarios in the image relevant to the query?

\begin{itemize}
    \item 0: The model completely misinterprets the image or fails to recognize key objects in the image relevant to the query.
    \item 1: The model partially misinterprets the image or recognizes some but not all key elements.
    \item 2: The model correctly interprets the image and identifies key elements.
\end{itemize}


\noindent \textbf{Response Accuracy}: Does the response provide factually correct information? Does it Hallucinate?

\begin{itemize}
    \item 0: The response contains factually incorrect information or even partially incorrect information.
    2: The response provides factually accurate information.
\end{itemize}


\noindent \textbf{Relevance}: Does the response address the user's query effectively?
\begin{itemize}
    \item 0: The response is not at all relevant to the query.
    \item 1: The response is somewhat relevant but may contain extraneous or slightly off-topic information.    
    \item 2: The response is directly relevant and focused on the user's query.
\end{itemize}

\noindent \textbf{Coherence and Fluency}: Is the model's response linguistically fluent and logically coherent?

\begin{itemize}
    \item 0: The model's response is either irrelevant, inconsistent with the query, or includes grammatically incorrect sentences.
    \item 1: The model's response is mostly relevant and grammatically correct, but there may be minor issues with coherence, style, or fluency.
    \item 2: The model's response is fully coherent, fluent, grammatically correct, and stylistically appropriate, given the query and context.
\end{itemize}

\noindent \textbf{Conciseness}:  Does the response answer the question concisely? I.e. Succinct, clear, and straight to the point without adding extraneous details

\begin{itemize}
    \item 0: The response either doesn't address the query adequately or is filled with a significant amount of extraneous information, making it lengthy and not concise.
    \item 1: The response addresses the query but includes some extra information that, while relevant, isn't essential to answering the question. The added details may provide context but aren't strictly necessary.
    \item 2: The response directly answers the query in a clear and succinct manner, providing only the information necessary to fulfill the user's request without any extraneous details.
\end{itemize}

\noindent \textbf{Completeness}: Does the response fully answer the query?

\begin{itemize}
    \item 0: The response does not answer the query.
    \item 1: The response partially answers the query, but leaves important questions or aspects unanswered.
    \item 2: The response fully answers the query, leaving no important aspects unanswered.
\end{itemize}

\noindent \textbf{Integrity}: Does the response show any harmful or offensive language or signs of unjust or prejudiced treatment related to characteristics such as race, age, gender, nationality, etc.?

\begin{itemize}
    \item 0: The response shows some sign of bias or harmful/offensive language.
    \item 2: The response shows no signs of bias or harmful/offensive language.
\end{itemize}










\subsection{Data Augmentation Prompts}\label{prompt:llava}
<s> [INST] <<SYS>>
You are an AI visual assistant that can analyze a single image. You receive five sentences, each describing the same image you are observing. In addition, specific object locations within the image are given, along with detailed coordinates. These coordinates are in the form of bounding boxes, represented as (x1, y1, x2, y2) with floating numbers ranging from 0 to 1. These values correspond to the top left x, top left y, bottom right x, and bottom right y.

The task is to use the provided caption and bounding box information, create a plausible question about the image, and provide the answer in detail.

Create complex questions beyond describing the scene.
To answer such questions, one should require first understanding the visual content, then based on the background knowledge or reasoning, either explain why the things are happening that way, or provide guides and help to user's request.  Make the question challenging by not including the visual content details in the question so that the user needs to reason about that first.

Instead of directly mentioning the bounding box coordinates, utilize this data to explain the scene using natural language. Include details like object counts, position of the objects, relative position between the objects.  

When using the information from the caption and coordinates, directly explain the scene, and do not mention that the information source is the caption or the bounding box.  Always answer as if you are directly looking at the image.
<</SYS>>
A young man smiles while wearing several ties.    tie: [0.574, 0.298, 0.752, 0.704]  tie: [0.464, 0.339, 0.639, 0.789]  tie: [0.349, 0.363, 0.563, 0.732]  tie: [0.259, 0.255, 0.668, 0.805]  person: [0.019, 0.065, 0.962, 0.988]  person: [0.0, 0.24, 0.214, 1.0]  tie: [0.316, 0.778, 0.443, 0.867]  tie: [0.386, 0.707, 0.496, 0.801]  tie: [0.251, 0.354, 0.402, 0.747]  tie: [0.44, 0.318, 0.63, 0.397]  tie: [0.566, 0.33, 0.655, 0.543]  tie: [0.25, 0.409, 0.359, 0.556] 
[/INST] 
Question:  What is unusual about this photo?  ===  Answer:  In the photo, the man is wearing a total of ten ties around his neck. This is considered unusual because it is not common for someone to wear multiple ties at once. In a typical setting, a person would wear only one tie. The man's goofy facial expression also adds to the unconventional and humorous nature of the image. </s><s>

[INST] 
A group of people standing outside of a black vehicle with various luggage.    person: [0.681, 0.242, 0.774, 0.694]  person: [0.63, 0.222, 0.686, 0.516]  person: [0.444, 0.233, 0.487, 0.34]  backpack: [0.384, 0.696, 0.485, 0.914]  backpack: [0.755, 0.413, 0.846, 0.692]  suitcase: [0.758, 0.413, 0.845, 0.69]  suitcase: [0.1, 0.497, 0.173, 0.579]  bicycle: [0.282, 0.363, 0.327, 0.442]  car: [0.786, 0.25, 0.848, 0.322]  car: [0.783, 0.27, 0.827, 0.335]  car: [0.86, 0.254, 0.891, 0.3]  car: [0.261, 0.101, 0.787, 0.626]
[/INST] 
Question:  What challenges do these people face?  ===  Answer:  In the image, a group of people is standing outside a black SUV in a parking area, surrounded by various pieces of luggage, including suitcases and backpacks. They are facing the challenge of fitting all their luggage into the black SUV. There are multiple suitcases and backpacks to be packed, which suggests that the group has a significant amount of belongings to accommodate. They might have to strategize and arrange the luggage efficiently to ensure that everything fits properly into the vehicle. Additionally, they need to consider the comfort of the passengers and visibility while driving, so the placement of the luggage must not obstruct the driver's view or make the passengers uncomfortable during the trip.</s><s>

[INST] 
A red fire hydrant is deep in the snow.    fire hydrant: [0.326, 0.612, 0.426, 0.72]
[/INST]
Question:  What challenges might this city face?  ===  Answer:  The city faces challenges due to the harsh winter conditions and heavy snowfall. In the image, a red fire hydrant is almost buried deep in the snow, which indicates the significant amount of snow the city has experienced. This can lead to various challenges such as difficulties in transportation, increased risk of accidents, and disruptions to daily life. For example, the recently plowed sidewalk near the fire hydrant shows that the city has to constantly clear snow from roads and sidewalks to maintain access and safety for pedestrians and vehicles. Moreover, emergency services, like firefighters, might face challenges accessing crucial equipment, such as fire hydrants, during emergencies due to the snow accumulation. This highlights the importance of effective snow management strategies and preparedness in such cities to minimize the impact of harsh winter conditions on residents and essential services.

[INST] 
A man with a red helmet on a small moped on a dirt road.    motorcycle: [0.561, 0.406, 0.176, 0.593]  person: [0.531, 0.062, 0.240, 0.835]   person: [0.737, 0.480, 0.056, 0.134]  bicycle: [0.759, 0.509, 0.048, 0.097]
[/INST]
% \zltodo{mention what prompts we use overall, and for specific tasks.}















What jacket would go well with this?

A navy blazer would look great with this shirt. The navy color will complement the shirt's blue hue, and the blazer will add a more formal touch to the outfit.

-

What cocktails can I make with these ingredients?

Here are some ideas: 1) A classic vodka sour. 2) An orange blossom martini, with vodka, triple sec, and freshly-squeezed orange juice.

-

Write a poem about this image in the style of Edgar Allen Poe.

In the snowy mountains,
a lone figure stands,
Gazing out at the frozen landscape's expanse. …

-

How long does this river go?

The river in the image is the Arno River, which flows through Florence, Italy. It stretches for approximately 241 kilometers (150 miles) and empties into the Ligurian Sea.

-

Describe this image in detail.

Four people are gathered around a campfire in the woods. They're all wearing casual outdoor clothing and sitting on chairs. There's a tent pitched nearby, and various camping gear scattered about.

-

(Given the motion signals)  Write a social media caption for this view.

Pedaling along the San Francisco Bay, taking in breathtaking views of the Golden Gate Bridge! The salty sea breeze invigorates me as I make my way to my next destination.

Do you have a trail recommendation?

A popular bike route is the Oakland Waterfront Bike Path, which runs along the East Bay coast from Jack London Square.


-

Write a poem with this sound.

Amidst the vast expanse, waves embrace, Dancing to the rhythm, in endless chase. Whispers of the sea, a soothing song, Ocean's waves, where dreams belong.


(Given the motion signals) Reply to my friend that I’ll call later.

“Hey! I’m running right now, so I won’t be able to answer now. I’ll call back later.”

==> sections/ethics.tex <==


We hereby acknowledge that all of the co-authors of this work are aware of the provided \textit{ACL Code of Ethics} and honor the code of conduct.
We state the ethical considerations and the potential impact to the community as follows.
\textbf{Datasets.}

\textbf{Applications.}

\textbf{Techniques.}


==> tables/tab_aac_archive.tex <==
\begin{table}[t]
\centering
    \scalebox{0.99}{
        \begin{tabular}{ccccc}
        \toprule
        \multirow{2}{*}{\textbf{Models}} &  \multicolumn{3}{c}{\textbf{AudioCaps}} \\ 
            \cmidrule(r){2-4}
          & CIDEr & SPICE & SPICEr \\  
        \midrule
        \midrule
        %Top Down-AlignedAtt(1NN) \cite{kim2019audiocaps} & 59.3 &  14.4 & 36.9 \\
        \multicolumn{1}{l}{TopDown-AlignedAtt} \cite{kim2019audiocaps} & 59.3 &  14.4 & 36.9 \\
        \multicolumn{1}{l}{CNN10-VGG} \cite{xu2021investigating} & 66.0  & 16.8 & 41.4 \\
        %Audio Captioning Transformer  \cite{mei2021audio} & 67.9 &  16.0 & 42.0 \\
        \multicolumn{1}{l}{ACT} \cite{mei2021audio} & 67.9 &  16.0 & 42.0 \\
        \multicolumn{1}{l}{PANNs + BERT} \cite{liu2022leveraging} & 66.7 & 17.2 & 42.0 \\
        %UnIVAL \cite{shukor2023unified} & 71.3  & 17.8 & 44.6 \\
        %Pengi \cite{deshmukh2023pengi} & 75.2  & 18.2 & 46.7 \\
        \midrule
        \multicolumn{1}{l}{\mn 7B (CLAP)} & 70.4  & 21.0 & 45.7 \\
        \multicolumn{1}{l}{\mn 13B (CLAP)} & \underline{72.1} & \underline{22.0} & \underline{47.0} \\
        \multicolumn{1}{l}{\mn 70B (CLAP)} & \textbf{77.8} & \textbf{23.0} & \textbf{50.4} \\
        %\midrule
        %Human \cite{kim2019audiocaps} & 91.3  & 21.6 & 56.5 \\
        \bottomrule
        \end{tabular}
    }
%\vspace*{\captionReduceTop}
%\vspace{-8pt}
\caption{
    \textbf{Zeroshot \underline{Audio} Captioning} results on AudioCaps. Ablations (bottom) over our \mn with varying base LLMs and sizes.
    \mn attains the best performance across multiple metrics, showing the model's strong performance in audio signal understanding.
    %Metrics: CIDEr, SPICE, SPICEr.
    %Baselines used (top): CRNN-R-DCASE \cite{xu2020crnn}, NCC (Neural Conditional Captioning) \cite{xu2022diversity}.
}
%\vspace*{\captionReduceBot}
%\vspace{-6pt}   
\label{tab:aac}
\end{table}




==> tables/tab_coco.tex <==
\begin{table}[t]

    \centering
    \scalebox{0.99}{
        \begin{tabular}{@{}ccc@{}}
        \toprule
        \multirow{2}{*}{\textbf{Models}} &  \multicolumn{2}{c}{\textbf{COCO}} \\ 
            \cmidrule(r){2-3}
          & CIDEr & BLEU-4 \\  
        \midrule
        \midrule
        \multicolumn{1}{l}{CM3Leon}    & 61.6 & -\\
        \multicolumn{1}{l}{OpenFlamingo-v2}    & 65.5 & - \\
        \multicolumn{1}{l}{Flamingo-80B}    & 84.3 & - \\
        \multicolumn{1}{l}{IDEFICS-9B}    & 46.0 & - \\
        \multicolumn{1}{l}{IDEFICS-80B}    & 91.8 & - \\
        \midrule
        % \multirow{3}{1.0cm}{\mn} & (Guanaco-33B)  & \textbf{57.8} & xx & xx & xx  \\
        \multicolumn{1}{l}{\mn (Guanaco-33B)} & xx & - \\
         \multicolumn{1}{l}{\mn (LLaMA2-13B)}  & 88.4 & \textbf{24.6} \\
         \multicolumn{1}{l}{\mn (LLaMA2-70B)}   & \textbf{91.1} & - \\
        \bottomrule
        \end{tabular}
    }
    %\vspace*{\captionReduceTop}
    %\vspace{-4pt}
     \caption{
            Zeroshot image captioning performance on COCO. Baselines used (top): CM3Leon, OpenFlamingo-v2-9B \cite{openflamingo}, Flamingo-3,9,80B \cite{flamingo}. Ablations (bottom) over our \dn with varying base LLMs and sizes.
        }
    %\vspace{-6pt}
    %\vspace*{\captionReduceBot}
    %\vspace*{-4pt}
    \label{tab:exp:coco}    
\end{table}

==> tables/tab_dataset_statistics.tex <==
\begin{wraptable}{r}{6cm}
%\begin{table}[t]
\centering
\scalebox{1.00}{
    \begin{tabular}{@{}cclcc@{}}
    \toprule
    \textbf{Modality} & \textbf{Dataset} & \textbf{\# Samples}  \\
    \midrule
    \midrule
    \multirow{1}{*}{Image\hspace{-5pt}} & LAION & 2B \\
    \midrule
    \multirow{1}{*}{Video\hspace{-5pt}} & HowTo100M & 100M  \\
    \midrule
    \multirow{2}{*}{Audio\hspace{-5pt}} & AudioSet & 2.1M \\
                                        %& Freesound & 600K \\    
                                        %& EpicAUDIO & 76K  \\
                                        %& AudioCaps & 46K  \\      
                                        %& MACS & 4K  \\
                                        & CLOTHO & 5K  \\
    \midrule
    \multirow{1}{*}{IMU\hspace{-5pt}} & Ego4D & 502K  \\
    \bottomrule
    \end{tabular}
}
%\vspace*{\captionReduceTop}
%\vspace{-8pt}
\caption{
    Statistics for the dataset used for alignment pre-training per each modality.
}
%\vspace*{\captionReduceBot}
%\vspace{-6pt}   
\label{tab:dataset_statistics}
%\end{table}
\end{wraptable}

==> tables/tab_exp_example.tex <==
\begin{table}[t]

    \centering
    \scalebox{0.85}{
        \begin{tabular}{@{}rrcccc@{}}
        \toprule
        & \multirow{2}{*}{\textbf{Models}} &  \multicolumn{2}{c}{\textbf{VQAv2}} & \multicolumn{2}{c}{\textbf{Data 2}} \\ 
            \cmidrule(r){3-4}
            \cmidrule(r){5-6}
          & & 0-shot    & $k$-shot & F1 & Acc. \\  
        \midrule
        \midrule
        \multicolumn{2}{r}{Baseline}    & 23.23 & xx & xx & 76.11  \\
        \midrule
        \multirow{3}{1.4cm}{\mn} & + Zeroshot                  & 19.39 & 23.08 & 18.46 & 21.52  \\
        & + Probing                   & 40.55 & 61.46 & \textbf{62.52} & \textbf{83.54}  \\
        & + Fine tuning               & 43.07 & \textbf{65.87} & 61.77 & 82.31 \\
        \midrule
        \multirow{3}{1.4cm}{\mn} & + Zeroshot                  & 31.89 & 36.38 & \multicolumn{2}{c}{\multirow{3}{*}{N/A}}    \\
        & + Probing                   & 45.12 & 58.01 &     \\
        & + Fine tuning               & \textbf{45.15} & 63.14 &     \\          
        \bottomrule
        \end{tabular}
    }
    %\vspace*{\captionReduceTop}
    %\vspace{-4pt}
     \caption{
            Caption goes here. 
        }
    %\vspace{-6pt}
    %\vspace*{\captionReduceBot}
    %\vspace*{-4pt}
    \label{tab:exp:example}    
\end{table}

==> tables/tab_human_eval_archive.tex <==
\begin{table}[t]
\centering
\scalebox{0.95}{
    \begin{tabular}{@{}lccc@{}}
    \toprule
    \textbf{vs. Human} & \textbf{Win} & \textbf{Tie} & \textbf{Lose}  \\
    \midrule
    \midrule
    OpenFlamingo & xx & xx & xx \\
    Mini-GPT4 & xx & xx & xx \\
    LLaVA & xx & xx & xx \\
    \midrule
    \mn (Guanaco-33B) & 24.9 & 15.0 & 60.0 \\
    \mn (LLaMA-2-70B) & 35.5 & 18.3 & 46.2 \\
    \bottomrule
    \end{tabular}
}
%\vspace*{\captionReduceTop}
%\vspace{-8pt}
\caption{
    \textbf{Visual reasoning} human evaluation results on pairwise comparisons (\% win, tie and lose) with ground-truth samples from \dn.
    Baselines used (top): OpenFlamingo-v2-9B \cite{openflamingo}, Mini-GPT4 \cite{minigpt4}, LLaVA \cite{llava}.
}
%\vspace*{\captionReduceBot}
%\vspace{-6pt}   
\label{tab:human_eval}
\end{table}

==> tables/tab_qual_examples_archive.tex <==

%% Non-licensed image, hence removing

    \toprule
    \multirow{2}{*}{\textbf{Example 2. How-To}} \\ \\
    \midrule
    \midrule
    \textbf{Input Image} &
        \begin{minipage}{.6\textwidth}
            \includegraphics[height=40mm]{figures/examples/warped_board.png}
            \vspace{2pt}
        \end{minipage}
    \\
    \textbf{Prompt} & \textbf{\textit{How do I fix it?}} \\
    \midrule    
    BLIP-2 & How do I fix a splinter in a wood deck?  \\
    \cmidrule(r){2-2}
    InstructBLIP & sand it \\
    \cmidrule(r){2-2}    
    Mini-GPT4 & It looks like the wood is rotting and needs to be replaced. You can try to remove the rotted wood and replace it with new wood.  \\
    \cmidrule(r){2-2}
    OpenFlamingo & I fix it by putting a new piece of wood on top of the old one. \\
    \cmidrule(r){2-2}
    LLaVA & To fix the wooden plank that is missing a portion, you need to create a new wooden support piece. In the image, you can see a long piece of wood, which can be cut into two sections to fit on either side of the broken (...) \\
    \midrule
    \mn 70B &  To fix a warped board on the floor, you can try to flatten it by placing heavy objects or weights on top of it and leaving them there for several hours. If that doesn't work, consider replacing the board entirely with a new one. \\
    

==> tables/tab_vqa_archive.tex <==
\begin{table}[t]

    \centering
    \scalebox{0.99}{
        \begin{tabular}{@{}cccc@{}}
        \toprule
        \multirow{2}{*}{\textbf{Models}} &  \multicolumn{1}{c}{\textbf{Hateful Meme}} &  \multicolumn{1}{c}{\textbf{VQAv2}} & 
        \multicolumn{1}{c}{\textbf{TextVQA}}\\ 
            \cmidrule(r){2-2}
            \cmidrule(r){3-3}
            \cmidrule(r){4-4}
          & AUC & Accuracy & Accuracy \\  
        \midrule
        \midrule
        \multicolumn{1}{l}{CM3Leon} \cite{cm3leon} & -  & 47.6 & -\\
        \multicolumn{1}{l}{OpenFlamingo-v2} \cite{openflamingo} & 51.6  & 50.5 & 24.2 \\
        \multicolumn{1}{l}{Flamingo-3B} \cite{flamingo}  & - & 49.2 & - \\
        \multicolumn{1}{l}{Flamingo-9B} \cite{flamingo}  & - & 51.8 & 31.8 \\
        \multicolumn{1}{l}{Flamingo-80B} \cite{flamingo}  & 46.4 & 56.3 & 35.0\\
        \multicolumn{1}{l}{IBELICS-9B} \cite{idefics} & 51.8  & 50.9 & 25.9\\
        \multicolumn{1}{l}{IBELICS-80B} \cite{idefics} & 60.6 & 60.0 &  30.9 \\
        \midrule
        % \multirow{3}{1.0cm}{\mn} & (Guanaco-33B)  & \textbf{57.8} & xx & xx & xx  \\
        % \multicolumn{1}{l}{\mn (Guanaco-33B)} & - & 57.8 \\
         \multicolumn{1}{l}{\mn 13B (ViT-G)} & 66.0 & 59.6 & 24.7 \\
         \multicolumn{1}{l}{\mn 70B (ViT-L)} & 68.2 & 62.0 & \textbf{35.4} \\
         \multicolumn{1}{l}{\mn 70B (ViT-G)} & \textbf{69.1} & \textbf{64.2} & 32.9 \\
        \bottomrule
        \end{tabular}
        }

    %\vspace*{\captionReduceTop}
    %\vspace{-4pt}
     \caption{
            \textbf{Zeroshot \underline{image}-based QA} accuracy on Hateful Meme, VQAv2, and TextVQA. Ablations (bottom) over \mn with varying base ViTs and LLM sizes.
            \mn demonstrates competitive zeroshot multimodal reasoning capabilities, compared to the baseline vision-language models.
        }
    %\vspace{-6pt}
    %\vspace*{\captionReduceBot}
    %\vspace*{-4pt}
    \label{tab:exp:vqa}    
\end{table}



==> tables/tab_vqa_wo_lora.tex <==






\begin{table}[t]

    \centering
    \scalebox{0.91}{
        \begin{tabular}{@{}ccccccc@{}}
        \toprule
        \multirow{2}{*}{\textbf{Models}} &  \multicolumn{1}{c}{\textbf{H-Meme}} &  \multicolumn{1}{c}{\textbf{VQAv2}} & 
        \multicolumn{1}{c}{\textbf{TextVQA}} & \multicolumn{1}{c}{\textbf{S-QA}}  & \multicolumn{1}{c}{\textbf{VizWiz}}  & \multicolumn{1}{c}{\textbf{OKVQA}}\\ 
            \cmidrule(r){2-2}
            \cmidrule(r){3-3}
            \cmidrule(r){4-4}
            \cmidrule(r){5-5}
            \cmidrule(r){6-6}
            \cmidrule(r){7-7}
          & AUC & Accuracy & Accuracy & Accuracy & Accuracy & Accuracy\\  
        \midrule
        \midrule
        %\multicolumn{1}{l}{CM3Leon} \cite{cm3leon} & -  & 47.6 & - & - & \textbf{37.6} & 23.8\\
        \multicolumn{1}{l}{OpenFlamingo-v2} \cite{openflamingo} & 51.6  & 50.5 & 24.2 & - & 27.5 & 37.8 \\
        \multicolumn{1}{l}{Flamingo-3B} \cite{flamingo}  & 53.7 & 49.2 & 30.1 & - & 28.9 & 41.2\\
        \multicolumn{1}{l}{Flamingo-9B} \cite{flamingo}  & 57.0 & 51.8 & 31.8 & - & 28.8 & 44.7\\
        \multicolumn{1}{l}{Flamingo-80B} \cite{flamingo}  & 46.4 & 56.3 & \underline{35.0} & - & 31.6 & \textbf{50.6}\\
        \multicolumn{1}{l}{BLIP-2 (FlanT5$_{\texttt{XXL}}$)} \cite{blip2}  & 52.0 & \textbf{65.0}$^\dagger$ & 44.1$^\dagger$* & 64.5 & 29.4 & \underline{45.9} \\
        \multicolumn{1}{l}{InstructBLIP (V-13B)} \cite{instructblip}  & 53.7 & - & 50.7$^\dagger$* & \underline{70.6} & 33.4 & - \\
        \multicolumn{1}{l}{IBELICS-9B} \cite{idefics} & 51.8  & 50.9 & 25.9 & - & \underline{35.5} & 38.4\\
        \multicolumn{1}{l}{IBELICS-80B} \cite{idefics} & 60.6 & 60.0 &  30.9 & - & \textbf{36.0} & 45.2 \\
        \midrule
        % \multirow{3}{1.0cm}{\mn} & (Guanaco-33B)  & \textbf{57.8} & xx & xx & xx  \\
        % \multicolumn{1}{l}{\mn (Guanaco-33B)} & - & 57.8 \\
         \multicolumn{1}{l}{\mn 13B (ViT-G)} & 66.0 & 59.6 & 24.7 & 52.7 & 24.4 &  33.1\\
         \multicolumn{1}{l}{\mn 70B (DINO-V2)} & 65.6 & 59.2 & 13.7 & - & 23.6 & 41.4 \\
         \multicolumn{1}{l}{\mn 70B (ViT-L)} & \underline{68.2} & 62.0 & \textbf{35.4} & 67.2 & 32.2 & 41.2 \\
         \multicolumn{1}{l}{\mn 70B (ViT-G)} & \textbf{69.1} & \underline{64.2} & 32.9 & \textbf{70.8} & 33.8 & 42.6 \\      
        \bottomrule
        \end{tabular}
        }

    %\vspace*{\captionReduceTop}
    %\vspace{-4pt}
     \caption{
            \textbf{Zeroshot \underline{Image}-based QA} results on 6 different VQA datasets (H-Meme: Hateful Meme, S-QA: Science QA).
            Ablations (bottom) over \mn with varying base ViTs and LLM sizes.
            \textbf{Bold} and \underline{underlined} denote the top and the second-best performance, respectively.
            \mn demonstrates competitive zeroshot multimodal reasoning capabilities, compared to the baseline vision-language models.
            *: Results with additional OCR inputs.
            $\dagger$: in-domain images (\ie COCO Caption, TextCap) have been used during training, thus not a strict zeroshot performance.            
        }
    %\vspace{-6pt}
    %\vspace*{\captionReduceBot}
    %\vspace*{-4pt}
    \label{tab:exp:vqa}    
\end{table}
